Shoring Up the Foundations: Fusing Model Embeddings and Weak Supervision

Foundation models offer an exciting new paradigm for constructing models with out-of-the-box embeddings and a few labeled examples. However, it is not clear how to best apply foundation models without labeled data. A potential approach is to fuse foundation models with weak supervision frameworks, which use weak label sources -- pre-trained models, heuristics, crowd-workers -- to construct pseudolabels. The challenge is building a combination that best exploits the signal available in both foundation models and weak sources. We propose Liger, a combination that uses foundation model embeddings to improve two crucial elements of existing weak supervision techniques. First, we produce finer estimates of weak source quality by partitioning the embedding space and learning per-part source accuracies. Second, we improve source coverage by extending source votes in embedding space. Despite the black-box nature of foundation models, we prove results characterizing how our approach improves performance and show that lift scales with the smoothness of label distributions in embedding space. On six benchmark NLP and video tasks, Liger outperforms vanilla weak supervision by 14.1 points, weakly-supervised kNN and adapters by 11.8 points, and kNN and adapters supervised by traditional hand labels by 7.2 points.

==> tables/main_coverage.tex <==
%!TEX root = ../main.tex

\begin{table*}[t]
    \centering
    \begin{tabular}{@{}rccccccccccc@{}}
        \toprule
        \multicolumn{1}{c}{} & \multicolumn{3}{c}{NLP (GPT-3)} & \multicolumn{3}{c}{Video (CLIP)} \\
        \cmidrule(l){2-4} \cmidrule(l){5-7}
        & \spam & \weather & \spouse & \basketball & \commercial & \tennis \\
        \textbf{WS-LM} average LF coverage
        & 16.2  & 8.8      & 3.8     & 49.2        & 54.5        & 66.9  \\
        \textbf{\sysname} average LF coverage
        & 61.7  & 99.0      & 15.9     & 57.5        & 73.3        & 99.4  \\
        \cmidrule(l){2-7}
        \textbf{\sysname\ vs. WS-LM}
        & +11.4  & +20.0     & +5.2    & +41.7        & +5.1        & +1.3  \\
        \bottomrule
    \end{tabular}
    \caption{
    \sysname\ improves over WS-LM by improving average coverage of the labeling
    functions. \todo{Put this into Table 1}
    }
    \label{table:coverage}
\end{table*}


==> tables/smoothness.tex <==
%!TEX root = ../main.tex

\begin{figure*}[t!]
    \centering
    \begin{minipage}{2in}
        \begin{flushright}
            \small
            \begin{tabular}{lr}    
                \toprule                                                     
                \textbf{Prompting} & F1-score \\
                \midrule
                No Prompt          & 48.5  \\
                Prompt at Beginning          & 50.2  \\
                \textbf{Prompt at End}          & \textbf{52.2} \\
                \bottomrule
            \end{tabular}
        \end{flushright}
    \end{minipage}
    \begin{minipage}{4.65in}
        \centering
        \includegraphics[width=4.5in]{figs/text_lipschitzness.pdf}
    \end{minipage}
    \caption{Left: Performance of using no prompting, prompting before, and prompting after for GPT-3 embeddings in \sysname\ for \spouse.
    Right: measures of smoothness of each prompting method on \spouse. \todo{Fix legends}}
    \label{smoothness-text}
\end{figure*}

